CoSMo: A Compact Spectral Space of Body Motion in Video

We introduce CoSMo, a compact spectral space of body motion in video, in which each motion is a single code that can be compared and edited without training, transferred to a new subject, interpolated, composed, scaled in intensity and detail, or sampled anew. Our encoder expresses how a clip's DINOv2 features change over time in a fixed temporal basis, the discrete cosine transform (DCT), and compresses this change into 384 numbers. Because each frequency band is the same cosine pattern in every code, codes are aligned in time, ordered from coarse to fine, and can be blended or added without matching frames. What stays constant over a clip cancels, and keeping fewer frequencies leaves less of the performer and scene. The encoder is trained on real videos and on synthetic motions of several characters, and lightweight adapters let a frozen image-to-video model render any code with any subject. On unseen videos, our code ranks the same motion on other bodies higher than DisMo, a per-frame representation, while its nearest neighbors show the same performer about 40% less often with a seven times more compact code. In generation, without per-motion training, CoSMo transfers motion more faithfully than FlexiAct and a text-prompt baseline, at least as faithfully as DisMo on automatic metrics and clearly better between humanoid bodies, and its blends keep much more of both source motions than DisMo's. Users rank CoSMo first nearly twice as often as DisMo for motion transfer (59% vs. 30%), place it top-two 94% of the time, and prefer it in 76% of the interpolation comparisons.

==> figures/abl_hourglass.tex <==
\begin{figure}[t]
  \centering
  \leavevmode\input{figures/abl_hourglass_anim}%
  \vspace{-16pt}%
  \caption{\textbf{Temporal compression}, same moments.
  Top: a ballet jump on an hourglass; bottom: a centaur's bow on a scarecrow.
  Learned compression distorts the subject, pooled frames break it apart or fold it flat, and the DCT keeps it whole while it moves.}%
  \label{fig:abl_hourglass}
  \vspace{-14pt}
\end{figure}


==> latexmkrc <==
# main.tex and main_supp.tex read each other's labels (xr-hyper, \externaldocument).
# Before building one of them, bring the other up to date so its .aux exists
# (latexmk is incremental, so this is quick when nothing changed). Works on
# Overleaf, which compiles the main document as -jobname=output.
# XR_OTHER stops the nested build from starting another one.
my %xr_other = ('main' => 'main_supp', 'main_supp' => 'main');
if (!$ENV{XR_OTHER}) {
    for my $arg (@ARGV) {
        next unless $arg =~ m{^(.*/)?(main|main_supp)(\.tex)?$};
        my $dir = defined $1 ? $1 : '';
        local $ENV{XR_OTHER} = 1;
        system("latexmk -cd -pdf -interaction=batchmode \"$dir$xr_other{$2}.tex\" > /dev/null 2>&1");
        last;
    }
}


==> secs/conclusion.tex <==
\section{Conclusion}

We introduced \modelname{}, a compact spectral space of body motion in video. Each motion is a single code of 384 numbers, the temporal spectrum of how a clip's features change, in a fixed DCT basis. Its codes are aligned in time and ordered from coarse to fine, so motions can be blended, added, scaled and sampled without
matching frames. A frozen image-to-video model renders any code on any subject,
transferring motion at least as faithfully as per-frame baselines, clearly better between humanoid subjects, and more faithfully than per-motion ones. Blends keep the motion of both sources, which per-frame embeddings lose.

By construction, the code cannot register timing below one
latent frame, and generated videos
can soften sharp timing. Since every clip is resampled to 64 frames, a code describes a motion relative to its clip. The same squat done twice lands in higher bands than done once, absolute speed comes from the output length (Sec.~\ref{sec:conditioning}), and a blend does not align the phases of its two motions. Despite better robustness to camera shake (Sec.~\ref{sec:ablations}), strong camera motion in the source can still carry over into the result. Supp.\ Fig.~S4 shows failure cases. We mainly test with body motion, where the gain over per-frame methods is largest (body$\to$body, Table~\ref{tab:transfer}); however, Supp.\ Fig.~S3 also shows non-body motions. A learned
prior over the DCT codes is a natural next step, to keep blends on plausible motions
rather than straight lines between codes, and to find unusual but plausible novel codes
beyond a single Gaussian.


==> secs/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We test how well the motion space separates motion from appearance (Sec.~\ref{sec:exp_space}), whether a frozen generator reproduces a motion from the code alone, and whether operations on codes behave like operations on motions (Sec.~\ref{sec:exp_transfer}).

\input{figures/qual_adapt}%
\subsection{Setup}
\label{sec:setup}

\paragraph{Data.}
Our synthetic dataset has 1{,}704 animations, each rendered on 5 of 107 characters
(8{,}520 clips). Real video comes from IDEA400, part of Motion-X \cite{lin2023motionx} (12{,}037 clips), and
HAA500 \cite{chung2021haa500} (6{,}944 clips), resampled or cut to 64 frames.
The encoder reads them at $224 \times 224$, as a full frame and a tight crop around
the motion. Real clips train it only through
reconstruction (Sec.~\ref{sec:encoder}). The adapters train on all 3 sets
(details in the supplementary).

\vspace{-5pt}
\paragraph{Evaluation data.}
Test videos and images are unseen in training. The motion space is probed
on 253 segments of 59 real videos (the out-of-distribution, or OOD set) and on 2 \emph{motion grids}
generated with Wan2.2-T2V-A14B \cite{wan2025wan}, one prompt per clip. 6 characters
(people, a robot, a doll, an ogre) perform 12 simple motions in one and 12
two-step motions in the other (72 clips each). An LLM writes the prompts, asked only for different motions on different subjects (details in supplementary). Labels come from the prompts, so timing
and poses vary, and some two-step clips miss the prompted order.
As FlexiAct tunes for ${\sim}4$\,h per motion (H200), the baseline transfer comparison favors few motions on diverse targets. 12 source videos of different kinds (6 OOD and 6 two-step motion-grid clips) are rendered on 10 target
images from our 101 still images of people, animals, figures and objects. Interpolation is scored on 150 blends of two body motions from unseen videos, each on a target image. Its user study uses 10 motion pairs generated with Wan2.2-T2V-A14B, drawn at random.

\vspace{-5pt}
\paragraph{Baselines.}
For the motion space, we compare with DisMo's released motion extractor \cite{ressler2025dismo}, whose code is its full sequence of per-frame embeddings. For transfer, we compare with DisMo, FlexiAct \cite{zhang2025flexiact} and a text baseline; for interpolation, with DisMo. DisMo and FlexiAct use CogVideoX-5B \cite{yang2024cogvideox}, so we report \modelname{} on both Wan2.2 and CogVideoX-5B (Sec.~\ref{sec:impl}); the user study uses CogVideoX-5B. The text baseline is Wan2.2-TI2V-5B \cite{wan2025wan} without adapters. Its prompt describes the source motion in order: which body parts move, in which direction, how often and how fast. Qwen2.5-VL-32B \cite{bai2025qwen25vl} writes all prompts, and appearance prompts describe only the target image.

\subsection{Motion Space Analysis}
\label{sec:exp_space}

Following DisMo \cite{ressler2025dismo}, Table~\ref{tab:space} probes both motion spaces without generation, by nearest-neighbor retrieval on videos neither encoder saw in training. On the 2 motion grids (Sec.~\ref{sec:setup}),
\emph{cross-body} retrieval asks whether a clip's nearest neighbor among the other characters performs the same motion (R@1). mAP measures
how highly the 5 other characters' versions of the same motion rank. \emph{Same character} takes a clip's 5 nearest neighbors in its
grid and, among those performing another motion, counts the share showing the same character. Every character performs every
motion, so only appearance makes them close. On the OOD set, \emph{same video} is how often a segment's nearest neighbor comes from
its own source video, which shares the performer, clothing, scene and camera but not always the motion. Lower is better for both. Our code finds the same motion on another body in 3 of 4 cases and ranks its other versions higher than DisMo, with a
seventh of the numbers. Its nearest neighbors show the same character about $40\%$ less often ($22$--$25\%$ vs.\ $37$--$42\%$, chance is $17\%$)
and come from the same video less often ($57\%$ vs.\ $74\%$).
\input{tables/space}
\input{tables/transfer}
\input{tables/ops_main}
\input{figures/qual_ops}%
\subsection{Motion Transfer and Interpolation}
\label{sec:exp_transfer}

On the 120 transfer pairs, we use DisMo's metrics, motion fidelity and temporal consistency, which depend on neither motion encoder.
\emph{Motion fidelity} follows Yatim \etal \cite{yatim2024space}: points are
tracked with CoTracker \cite{karaev2024cotracker} in both videos, each generated
track is matched to the source track whose frame-to-frame directions correlate
best with it, and the correlations are averaged. As our scope is the body's motion, we compute it
on tracks with camera motion removed and weight it by how far the subject moves relative to the source, capped at 1 (details in the supplementary).
\emph{Temporal consistency} is the CLIP \cite{radford2021learning} similarity of
consecutive frames, and \emph{image similarity} that of each frame to the target image. All metrics are computed on 25 evenly spaced frames of each video, the length of DisMo's output, which slightly favors DisMo (Supp.\ Table~S1). Confidence intervals (CI, 95\%) come from 10{,}000 bootstrap resamples of the pairs, or of the participants for the user study.
In Table~\ref{tab:transfer}, \modelname{} follows the source motion more closely than all baselines ($0.42$ on
CogVideoX and $0.41$ on Wan2.2, against $0.38$ for DisMo; $+0.04$ on CogVideoX, CI $[0.02, 0.07]$) at similar temporal consistency and image similarity, without per-motion training ($119$\,s per
video on CogVideoX and $40$\,s on Wan2.2, against $3.9$\,h for FlexiAct).
On 300 further body-motion samples from videos unseen in training (the OOD set, the two-step motion grid and other action clips),
DisMo scores $0.37$ against $0.38$ for \modelname{} on CogVideoX and $0.39$ on Wan2.2 (Table~\ref{tab:transfer}; $+0.01$ on CogVideoX, CI $[-0.01, 0.03]$). The gap is larger for the 107 that
transfer motion to a humanoid body (body$\to$body), which covers people but also figures with very distinct proportions, such as dolls, a paper boy or a scarecrow: $0.42$ and $0.42$ against $0.36$ ($+0.06$ on CogVideoX, CI $[0.03, 0.09]$). Although our cross-character pairs are synthetic, the gain carries over to the 100 OOD samples with real source videos ($+0.05$ on CogVideoX, CI $[0.01, 0.09]$). We attribute this to real videos making up $69\%$ of the training clips and to the small code, which leaves little capacity for appearance.


Automatic metrics miss how convincing a motion is, so we also run a user
study (Table~\ref{tab:transfer}; 29 participants for transfer and 27 for interpolation, 10 examples each; details in the supplementary). Users clearly prefer our method: they rank it first in $59\%$ of transfer answers (CI $[53\%, 66\%]$, chance $25\%$), $30$ points more often than DisMo (CI $[18, 41]$), and choose it in $76\%$ of interpolation answers (CI $[70\%, 82\%]$). On non-human targets, the preference is strongest ($76\%$ of first places), while on those of the 300 samples the motion score ties; Supp.\ Sec.~A explains why. In Fig.~\ref{fig:qual_adapt}, DisMo turns the golem's boulder into the doll's stretched head and keeps the mannequin facing forward instead of twirling. The text baseline and FlexiAct, whose prompts describe the source's action, add the boulder itself. Our generator never sees the source, so the mannequin twirls and the doll bends, keeping their own proportions.

For interpolation, we blend 2 codes (for DisMo, its embeddings frame by frame, Supp.\ Sec.~A gives its recipe and how a blend is scored). This changes the
motion steadily from one code to the other (Figs.~\ref{fig:teaser},
\ref{fig:qual_ops}). Our blends keep the motion of both sources, on average $64\%$ of its amount on CogVideoX against $40\%$ for DisMo,
whose blends lose much of it (Table~\ref{tab:transfer}; $+0.10$ on CogVideoX, CI $[0.07, 0.12]$), most clearly on the 71 blends onto a humanoid body
(body$\to$body: $0.37$ and $0.38$ against $0.24$; $+0.13$ on CogVideoX, CI $[0.10, 0.16]$).
The other operations of Sec.~\ref{sec:operations} behave as expected (Table~\ref{tab:ops_main}). We re-encode each generated video with our encoder and compare it with the 21 source codes: sums lie close to both motions, and codes cut to fewer bands still identify their source. On tracks, the subject's motion grows with $\alpha$ in every pair, and sampled codes are as temporally consistent as real transfers.

\section{Ablations}
\label{sec:ablations}


We ablate compression techniques, the temporal basis, and the encoder's design. Due to compute budget, ablations train from scratch for fewer steps than the final model.
\vspace{-8pt}
\paragraph{Temporal compression.}
Transfer is scored on body motion in 320 pairs from 51 unseen clips (30 real, 21 generated), 198 with a person or humanoid source (body$\to$all), 55 of them with a
humanoid target (body$\to$body). Learned queries compressing the clip's motion (learned compression) collapse the code. Its slots become near-copies, and 21
principal components hold $90\%$ of its variance (Table~\ref{tab:compression}). A low-pass filter averaging every 4 frames before the
transformer (pooled frames) follows body motion about as well as the DCT ($0.387$ vs.\ $0.382$), less closely when the target is a humanoid ($0.383$ vs.\ $0.415$, DCT $+0.033$, CI $[0.001, 0.060]$), and keeps the target
less well ($0.873$ vs.\ $0.885$; DCT $+0.012$, CI $[0.006, 0.019]$). It breaks the subject apart or folds it flat, while the DCT keeps it whole and moving
(Fig.~\ref{fig:abl_hourglass}). The DCT keeps a motion's \textit{essence} rather than copying the source frame by frame, with coarse-to-fine control for free (Fig.~\ref{fig:qual_ops}). It also copes better with camera shake, which pooled frames fold into
their slots. With the query shaken or vibrating by up to $3$--$4\%$ of the frame, cross-body R@1 on both grids, without Table~\ref{tab:space}'s random resizing, is $53\%$/$64\%$ for the DCT vs.\ $37\%$/$40\%$ for pooled frames, which lead only when clean ($68\%$ vs.\ $63\%$).\par%
\input{figures/qual_ours}
\vspace{-8pt}
\paragraph{Temporal basis.}
Without training, 16 of 64 DCT bands retain nearly as much motion as the best
fitted basis (Fig.~\ref{fig:why}a). Without a time axis (the same code at every frame), an
adapter barely moves the subject (motion fidelity $0.17$ vs.\ $0.33$, Supp.\ Sec.~B).
Fewer bands retain less appearance and video-specific detail, yet cross-body
retrieval holds down to 4 bands before dropping sharply (Fig.~\ref{fig:why}d).

\input{figures/abl_hourglass}
\input{tables/compression}
\vspace{-8pt}
\paragraph{Encoder design.}
Removing $\mathcal{L}_{\text{nce}}$ or replacing DINOv2 with RGB patches costs the most cross-body retrieval (R@1 $66\%$/$42\%$ against $75\%$), even on synthetic training pairs ($83\%$/$82\%$ against $100\%$). The per-frequency balance and the frame-0 subtraction mainly help on fast motions (mAP on the fastest third $0.455$ against $0.443$ and $0.435$) and keep less of what is specific to a video (same video $56\%$ against $62\%$ and $64\%$ without them, Supp.\ Table~S3).


==> secs/llm.tex <==
\section*{LLM Usage Statement}
Qwen2.5-VL-32B writes the motion and appearance prompts of the baselines (Sec.~\ref{sec:setup}), and an LLM (Claude)
writes the text prompts from which Wan2.2-T2V-A14B generates the motion grids and interpolation test clips. An LLM (ChatGPT) helped screen the user study's target images, flagging those whose shape cannot perform an articulated motion. For the research and writing, an LLM-based coding assistant (Claude Code) was used to help write code and run training scripts. LLMs were also used to draft, edit and refine the text and to help in generating figures in the paper. The authors reviewed all code, results and text, and take full
responsibility for the content of the paper.


==> secs/method.tex <==
\section{Method}
\label{sec:method}
Our aim is a compact code for the body motion in a video clip, largely independent of the performer's appearance and of the
clip's length, so that it can drive a frozen video diffusion model to render that motion with any subject.
To this end, a spectral encoder, trained with a decoder, compresses a clip's motion into a code $c \in \mathbb{R}^{M \times K}$ with $M = 24$
channels and $K = 16$ temporal frequencies (384 numbers; Fig.~\ref{fig:pipeline}a, Sec.~\ref{sec:encoder}). Lightweight adapters then
let the frozen model render the code with the subject of a still image (Fig.~\ref{fig:pipeline}b, Sec.~\ref{sec:conditioning}). The encoder is trained first, and the
adapters are then trained on its frozen codes. Operations on codes act on motions without further training
(Sec.~\ref{sec:operations}).

\input{figures/pipeline}

\subsection{Spectral Motion Encoder}
\label{sec:encoder}

\paragraph{Encoder.} 
%
All clips are resampled to $T=64$ frames, and each frame passes through a frozen DINOv2-B/14~\cite{oquab2024dinov2}, giving a $16\times16$ grid of patch features $g_t \in \mathbb{R}^{256\times768}$, $t=0,\dots,T-1$. A learned projection $P$ maps each feature to the transformer width of 384, and we subtract the first frame, $r_t = P(g_t)-P(g_0)$, so that what stays constant over the clip cancels. A temporal DCT at every patch keeps the $K=16$ lowest frequencies, $f_k = \frac{1}{T}\sum_t r_t B_{k,t}$ for $k<K$, where $B_{k,t}$ is the DCT basis over $T$ frames. A transformer with full attention processes the resulting $256\times K$ patch--frequency tokens. For each frequency $k$, its own learned query pools over the 256 patches, and a linear map projects the result to $M=24$ channels, giving column $c_{:,k}$. The code $c\in\mathbb{R}^{M\times K}$ acts as a pseudo-DCT of the motion. It is not the transform of any one signal, yet each column belongs to one frequency, ordered from slow to fast, and its inverse DCT gives $M$ trajectories over time.
\if 0
The encoder takes the DINOv2 features \cite{oquab2024dinov2} of a clip, expresses how
each patch's features change over time with a temporal DCT, and compresses that
spectrum into the code.
All clips are resampled to $T=64$ frames and each frame passes through a frozen
DINOv2-B/14, giving a $16\times16$ grid of patch features
$g_t \in \mathbb{R}^{256 \times 768}$, $t = 0,\dots,T-1$. A learned
projection $P$ maps each patch feature to the transformer width of 384, and we subtract the
first frame, $r_t = P(g_t) - P(g_0) \in \mathbb{R}^{256 \times 384}$, so that what
stays constant over the clip cancels.
A temporal DCT at every patch
keeps the $K = 16$ lowest frequencies,
$f_k = \frac{1}{T}\sum_{t} r_t B_{k,t}$ for $k < K$, where $B_{k,t}$ is the DCT
basis over $T$ frames.
This turns the clip into $256 \times K$ tokens indexed by patch and
frequency, which a transformer with full attention processes. For each
frequency $k$, its own learned query pools over the 256 patches into one
vector, and a linear map projects the result to $M = 24$ channels,
giving column $c_{:,k}$. The code $c \in \mathbb{R}^{M \times K}$, 384 numbers
in total, acts as a pseudo-DCT of the motion. It is not the transform of any one
signal, but each column belongs to one frequency, ordered from slow to fast, and its
inverse DCT gives $M$ trajectories over time.
\fi

\paragraph{Decoder.}
A decoder, used only in training, takes
the code and a first frame and predicts the DCT coefficients $\hat D_k$ of each
patch's displacement from the first frame, and the inverse DCT gives the features
$\hat g_t$ at every frame (Fig.~\ref{fig:pipeline}a).
The supplementary details both networks.

\paragraph{Training and losses.}
Both are trained jointly with
\[
  \mathcal{L} = \mathcal{L}_{\text{rec}} + \lambda_{\text{nce}}\,\mathcal{L}_{\text{nce}}
              + \lambda_{\text{reg}}\,\mathcal{L}_{\text{reg}}.
\]
The reconstruction loss $\mathcal{L}_{\text{rec}}$ compares predicted and true displacements from the first frame
through their DCT coefficients. Each frequency's error is divided by its own energy, which gives the fast
frequencies a boost, since the slowest one holds about half of the energy. We also add two auxiliary terms, found
empirically to refine the reconstruction: a squared error weighted toward patches that move, and a cosine distance
between the two displacements.

The reconstruction task depends on the data. In synthetic data the same motion is performed by several characters, so
reconstruction runs across characters. For clips $A$ and $B$ of the same motion, the
decoder receives $A$'s code and $B$'s first-frame features and must predict
$B$'s features at every frame, and symmetrically from $B$ to $A$. Real clips have no such pairs, so each is
seen in two augmented views, and the decoder predicts each view from the other view's code. $\mathcal{L}_{\text{nce}}$ is an InfoNCE loss over the synthetic codes of a batch, in which
the positive for each code is the other character's code of the same motion. It pulls
the codes of one motion together across bodies and pushes other motions away.
$\mathcal{L}_{\text{reg}}$ keeps the code's dimensions varied and decorrelated.

\subsection{Rendering with a Frozen Video Model}
\label{sec:conditioning}

We pair the encoder with a fully frozen Wan2.2-TI2V-5B \cite{wan2025wan} and trainable adapters, a mapping network and conditional LoRA layers. The training prompt is the same for
every clip, ``an articulated motion, high quality''. At inference, a description of the target's appearance is placed before it.

\paragraph{Inverse DCT and per-frame expansion.}
The code, normalized to a fixed norm, is expanded over the $F$ latent
frames of the output ($F = 16$ in training) with the inverse DCT (the same basis with $T = F$, so frequency $k$
means the same thing as in the encoder),
\[
  u_f = \sum_{k} c_{:,k} B_{k,f} \in \mathbb{R}^{M}, \qquad f = 0,\dots,F-1,
\]
where $B_{k,f}$ is the value of the $k$-th DCT cosine at latent frame $f$.
At other lengths, the cosines are sampled at $F$ evenly spaced latent frames, so the output length, not the source, sets the motion's absolute speed.
A mapping network (details in the supplementary) turns each $u_f$ into an embedding
$m_f \in \mathbb{R}^{768}$. We center its output with a running mean and a
running scale, fixed at test time. Without centering we found the network drifts
toward emitting the same embedding for every clip.
These per-frame embeddings come from the code alone, not from the source.

\paragraph{Conditional LoRA.}
We add a conditional LoRA \cite{hu2022lora,ressler2025dismo} to linear layers
throughout the transformer. For a frozen layer $y = Wx$ and a token $x$ in
latent frame $f$,
\[
  y = Wx + U\big[(1 + \gamma(m_f)) \odot Vx + \beta(m_f)\big],
\]
where $V$ and $U$ are the low-rank factors, and $\gamma$ and $\beta$ are
linear maps of the frame's motion embedding. $U$, $\gamma$ and $\beta$ start at zero, so training starts from the
unmodified model.

\paragraph{Training and sampling.}
We train the mapping network and LoRA with the flow-matching loss, replacing the code with a learned null code
for $10\%$ of samples, for classifier-free guidance \cite{ho2022classifier} between the code and the null code.
\subsection{Operations in the Motion Space}
\label{sec:operations}

Every operation below builds a code from unit-norm codes $\hat c = c / \lVert c \rVert$; nothing needs training or fine-tuning (Fig.~\ref{fig:qual_ops}).

As codes are vectors, motions can be combined through simple arithmetic.
The blend $(1-w)\,\hat c_A + w\,\hat c_B$, renormalized, \emph{interpolates} from motion
$A$ to motion $B$ (Fig.~\ref{fig:qual_ops}, Interp.\ row; Supp.\ Fig.~S1), and the sum $\hat c_A + \hat c_B$, the blend at $w = 0.5$ up to scale, \emph{composes} them (Fig.~\ref{fig:qual_ops}, $w = 0.5$; Supp.\ Fig.~S2).
The direction $d$ from the mean code of the $20\%$ stillest training clips to that of the $20\%$ most
moving ones controls \emph{intensity}: $\hat c + \alpha d$ turns a motion down ($\alpha < 0$) or up
($\alpha > 0$) (Fig.~\ref{fig:qual_ops}, Intensity row).

Keeping only the first $K' < K$ frequency bands gives a \emph{coarser} version of a
motion, its slow course without the fast detail, which sets how closely a target follows the source (Fig.~\ref{fig:qual_ops}, Coarse row).
Since even DCT bands are symmetric in time and odd ones are antisymmetric, negating
the odd columns approximately plays a motion backwards (Fig.~\ref{fig:why}c).

Finally, the space holds motions that no clip performed. Codes sampled from a Gaussian $\mathcal{N}(\mu, \Sigma)$ fitted to the unit
training codes are new motions. To push further from the data, we use novelty search \cite{lehman2011abandoning}.
Starting from real codes, we ascend novelty $\nu$, one minus the mean cosine similarity to the three nearest training codes,
penalized for leaving the support of the data (details in the supplementary), and keep a diverse subset of the most novel codes inside it. The supplementary gives more details and examples.

\subsection{Implementation Details}
\label{sec:impl}

We build on Wan2.2-TI2V-5B \cite{wan2025wan} as it generates different video lengths, keeps the target's aspect ratio and has 16 latent frames, one per band of our code. For the baseline comparisons, we also build on CogVideoX-5B-I2V \cite{yang2024cogvideox}, as both DisMo and FlexiAct build on it. The supplementary gives the architectures and training schedules.


==> tables/dct.tex <==
% Table dct (\label{tab:dct}), \input from secs/experiments.tex
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
 & DCT (ours) & pooled frames & PCA (fitted) \\
\midrule
energy kept, all 16 & $92.0 / 90.9$ & $89.9 / 89.0$ & $92.5 / 91.2$ \\
energy kept, first 4 & $\mathbf{76.3} / \mathbf{77.5}$ & $12.2 / 11.2$ & $78.4 / 79.2$ \\
energy kept, first 1 & $53.6 / 58.9$ & $0.6 / 0.4$ & $58.3 / 64.4$ \\
cross-character R@1 & $92.0$ & $92.0$ & $92.0$ \\
8-frame delay, all 16 & $0.70$ & $0.71$ & $0.70$ \\
8-frame delay, first 4 & $\mathbf{0.80}$ & $0.21$ & $0.78$ \\
\bottomrule
\end{tabular}
\caption{Temporal bases compared on the encoder's input, without training.
Energy kept: \% of the displacement of DINOv2 tokens that 16 (or the first 4,
or the first 1) coefficients per position reconstruct, on 150 held-out synthetic
clips / 16 real videos. PCA is fitted to the other half of the synthetic motions:
the best 16-dimensional temporal basis for this data. R@1: nearest other clip
is the same motion on another character (\%). Delay: cosine between a real
video's representation and that of the same video started eight frames later,
from all 16 or only the first 4 coefficients (16 real videos with at least 72
frames; between different videos: about $0.2$, and $0.10$ for the first four
pooled windows). Pooled frames: the mean of each of 16 windows of four frames.}
%% src: v26/eval/dct_probe/probe.json (v26/tools/dct_probe.py),
%%      v26/eval/dct_probe/probe2.json (v26/tools/dct_probe2.py)
\label{tab:dct}
\end{table}


==> tables/nodct.tex <==
% Table nodct (\label{tab:nodct}, also \label{tab:dct}), \input from secs/experiments.tex. Merged 2026-10-28 (user: put the temporal-basis
% table in the main paper, merged with Table 3); it replaces tables/dct.tex, which the supp no longer inputs.
% 2026-10-29 (user: "lets remove timebins" ... "until we can show a clear advantage over dct"): the pooled-frames row of (a)
%     removed: DCT 92.0 / 76.3 / .80 vs pooled frames 89.9 / 12.2 / .21. Restore from git (a36cb74) if the advantage is shown.
% (a) training-free basis probe on the encoder's input: v26/eval/dct_probe/probe.json (dct_probe.py, 150 held-out synthetic clips; PCA fitted
%     to the other half), delay from probe2.json (dct_probe2.py, 16 real videos >= 72 frames). Real-video energy (not shown): DCT 90.9/77.5,
%     pooled 89.0/11.2, PCA 91.2/79.2; delay with all 16: .70/.71/.70; cross-character R@1 92/92/92.
% (b) the no-DCT ablation (2026-10-27, user: "justify dct over just compressing"): DCT row = the matched arm m3_dct / ad_m3_dct (30k + 30k
%     from scratch, all three datasets); learned compression = m3_lc / ad_m3_lc (runpod/nodct, pod irv2524u9mvzin, running): --basis box
%     --pool_global 1, adapter --deep_time learned. Left EMPTY until it lands (user: "if there is an ablation running just leave its area
%     empty"). Motion fidelity: to be scored with the Table 2 metric on both arms' fixed transfers. DCT probes: space_table results.json
%     (m3_dct), grid_reframe (3 draws), eval/abl_haar_m3/lod.json (k = 4).
% (c) number of bands (added 2026-10-28, user: "add it"): the PAPER model's code (wan_hr encoder) cut to its first k bands,
%     v26/tools/space_table/trunc_probe.py -> trunc_ours.json (same numbers as fig:why b and the text). k=1: R@1 53, same 39, leak 32;
%     k=8: 79 / 53 / 30. The matched arm cut the same way: trunc_m3_dct.json (k=4: 73 / 46 / 34; k=16: 74 / 62 / 42).
% Motion fidelity in (b) and (d) (2026-10-28): Table 2's metric (Y6) via v26/tools/abl_y6/{masks,score}.py -> results.json, on the 40 fixed
%     transfers of best_choices.json minus 2 held-pose sources (toetouch_hold_3/6: no subject point moves > 5% of its height) = 38.
%     (b) DCT = ad_m3_dct .338. (d) Oct 8 adapters (20k steps from scratch on abl_dct codes): ad_dct .327 vs ad_static (--deep_time const)
%     .151, paired -.176 +- .032 (4/38 wins), 50% of ad_static outputs nearly still (gate < .05) vs 21%. ad_dct_plain .321.
%     Nearly-still column (still_share in results.json) added to (d) 2026-10-28 (user: "add it to table").
%     (The old -0.13 was the earlier subject-motion-v2 metric, ad_static vs ad_dct_plain.)
% 2026-10-30 (user: "from table 3 just remove (b) [... in table 4 now] and (c) [mentioned in fig 3]"): old (b) trained-from-scratch
%     probes and (c) bands-kept rows removed (Table 4 = tables/compression.tex, Fig. 3d); old (d) is now (b).
% Same day (user: "actually remove (b) too. i think its useless here"): the time-axis rows removed; their numbers stay in the text
%     (Ablations, Temporal basis; supp) without a table: over the frames .33 / 21% nearly still, same at every frame .15 / 50%.
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
\multicolumn{4}{l}{\emph{Basis on the encoder's input, no training}} \\
 & \multicolumn{2}{c}{energy kept\,$\uparrow$} & delay\,$\uparrow$ \\
 & all 16 & first 4 & first 4 \\
\midrule
DCT (ours)    & $92.0\%$ & $76.3\%$ & $\mathbf{0.80}$ \\
PCA (fitted)  & $92.5\%$ & $78.4\%$ & $0.78$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Why the DCT.} Share of the change of the encoder's
input (DINOv2 features, 150 held-out synthetic clips) kept by 16 or the first 4
coefficients per position; PCA is fitted to the data. Delay: cosine between the
first 4 coefficients of a video and of the same video started 8 frames later.}
\label{tab:nodct}
\label{tab:dct}
\end{table}


==> tables/ops_main.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{2pt}
\setlength{\aboverulesep}{1pt}\setlength{\belowrulesep}{1pt}\renewcommand{\arraystretch}{1.0}\setlength{\abovecaptionskip}{3pt}%
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lll@{}}
\toprule
operation & measure & result \\
\midrule
coarse to fine & source found among 21, $k < 2/4/8/16$ & $23/55/88/91\%$ \\
intensity & motion in body heights, $\alpha = -2 \rightarrow +2$ & $.05 \rightarrow 1.38$ \\
composition & cosine to A\,/\,B: A+B vs.\ the other alone & $.34/.33$ vs.\ $.06$ \\
sampling & temp.: sampled vs.\ same-target transfers & $.978$ vs.\ $.969$ \\
\bottomrule
\end{tabular*}
\caption{\textbf{Operations, measured} on 168 pairs, 105 sums, 210 samples (chance $5\%$; Supp.\ Table~S4).}
\label{tab:ops_main}
\vspace{-14pt}%
\end{table}


==> tables/temporal.tex <==
% Table temporal (\label{tab:temporal}), \input from secs/experiments.tex -- the matched arms (2026-10-12/13): encoder + adapter 30k each
% from scratch on synthetic + IDEA400 + HAA500, plain loss; src v26/eval/abl_motion/per_pair_m3.jsonl, v26/eval/abl_haar_m3/
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcc}
\toprule
 & DCT (ours) & per frame \\
\midrule
numbers per clip & 384 & 2{,}048 \\
motion fidelity\,$\uparrow$ & $0.347$ & $\mathbf{0.396}$ \\
motion kept, first 2 bands\,$\uparrow$ & $0.92$ & -- \\
motion kept, first 4 bands\,$\uparrow$ & $0.98$ & -- \\
\bottomrule
\end{tabular}
\caption{\textbf{Temporal representation} (Sec.~\ref{sec:supp_abl}). Motion
fidelity as in Table~2 (camera removed, weighted by the subject's motion) over 40 curated transfers. Motion kept: cosine
between the motion decoded from the first bands and from the full code.}
\label{tab:temporal}
\end{table}


==> tables/transfer.tex <==
\begin{table*}[t]
\centering
\setlength{\abovecaptionskip}{4pt}
\setlength{\tabcolsep}{1.5pt}
\providecommand{\dottedrow}[1]{\noalign{\vskip .4ex\hbox to #1{\leaders\hbox to 2pt{\hss\vrule height .4pt depth 0pt width .5pt\hss}\hfill}\vskip .65ex}}
\begingroup\footnotesize
\setlength{\aboverulesep}{1pt}\setlength{\belowrulesep}{1pt}\renewcommand{\arraystretch}{1.0}%
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccccccc}
\toprule
 & & & \multicolumn{4}{c}{transfer, 120 pairs} & \multicolumn{3}{c}{transfer, 300 pairs} & \multicolumn{2}{c}{body$\to$body, 107} & \multicolumn{3}{c}{interpolation, 150} & \multicolumn{2}{c}{body$\to$body, 71} \\[-.3ex]
\cmidrule(lr){4-7}\cmidrule(lr){8-10}\cmidrule(lr){11-12}\cmidrule(lr){13-15}\cmidrule(lr){16-17}
method & frames & time\,$\downarrow$ & mot.\,$\uparrow$ & temp.\,$\uparrow$ & img.\,$\uparrow$ & user 1st/top-2\,$\uparrow$ & mot.\,$\uparrow$ & temp.\,$\uparrow$ & img.\,$\uparrow$ & mot.\,$\uparrow$ & img.\,$\uparrow$ & mot.\,$\uparrow$ & temp.\,$\uparrow$ & user\,$\uparrow$ & mot.\,$\uparrow$ & temp.\,$\uparrow$ \\
\midrule
text baseline                       & 61 & $\mathbf{29}$\,s & $.256$ & $.971$ & $.854$ & $4/19$ & $.307$ & $.965$ & $.841$ & $.410$ & $.850$ & -- & -- & -- & -- & -- \\
FlexiAct \cite{zhang2025flexiact}   & 49 & $3.9$\,h & $.361$ & $.973$ & $.858$ & $7/19$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
DisMo \cite{ressler2025dismo}       & 25 & $53$\,s & $.378$ & $.982$ & $.908$ & $30/67$ & $.371$ & $.983$ & $.910$ & $.360$ & $.896$ & $.226$ & $\mathbf{.990}$ & $24\%$ & $.237$ & $\mathbf{.988}$ \\
\modelname{} (Cog-5B) & 49 & $119$\,s & $\mathbf{.421}$ & $\mathbf{.984}$ & $\mathbf{.917}$ & $\mathbf{59/94}$ & $.380$ & $\mathbf{.985}$ & $\mathbf{.918}$ & $.418$ & $\mathbf{.899}$ & $.322$ & $.987$ & $\mathbf{76\%}$ & $.370$ & $.983$ \\
\dottedrow{\textwidth}
\modelname{} (Wan-5B)       & 61 & $40$\,s & $.410$ & $.983$ & $.905$ & -- & $\mathbf{.394}$ & $.983$ & $.902$ & $\mathbf{.421}$ & $.888$ & $\mathbf{.348}$ & $.986$ & -- & $\mathbf{.384}$ & $.981$ \\
\bottomrule
\end{tabular*}
\endgroup
\caption{\textbf{Motion transfer and interpolation} (Sec.~\ref{sec:exp_transfer}). Mot.: motion fidelity; img.: CLIP
similarity to the target image. Time: per video on one H200, including any per-motion training but not the text baseline's captioning. User 1st/top-2: \% of
answers (user study, 10 examples) that rank the method first / first or second of the four. User (interpolation): share that choose the method of the two (user study, 10 pairs). Interpolation: in-between videos
($w = .25, .5, .75$), motion scored against both source motions. FlexiAct not run on 300 pairs.}
\label{tab:transfer}
  \vspace{-12pt}%
\end{table*}


==> tables/user.tex <==
% NOT USED since 2026-11-12: the user study is back in Table 2 (tables/transfer.tex), on the Cog-5B row.
% Table user (\label{tab:user}), \input from tables/transfer.tex: it sits to the right of Table 2 in the same full-width float (a separate single-column
% table pushed the conclusion onto a new page). Split out of Table 2 on 2026-11-08 (user: "remove user study from table 2 and put it as a new table
% somewhere else ... user study will now be done on cog"); the CoSMo row is CoSMo on CogVideoX-5B.
%% Results so far 2026-11-12 8:41 AM Vancouver (userstudies_build/fetch_responses.py + summarize_responses.py): share of FIRST choices.
%%   Transfer (v47): 10 participants, 100 answers: ours 63/100, DisMo 24, FlexiAct 8, text 5 (top-2: 96 / 61 / 23 / 20).
%%   Interpolation (v27): 9 participants, 90 answers: ours 67/90, DisMo 23 (transitions 30/45, compositions 37/45); one earlier-version
%%   participant (ours 8/10) left out. Study still open (42-submission cap each); update before submission.
\centering
\footnotesize
\setlength{\tabcolsep}{1pt}
\begin{tabular*}{\linewidth}{@{}l@{\extracolsep{\fill}}cc@{}}
\toprule
method & transfer$\uparrow$ & interp.$\uparrow$ \\
\midrule
text baseline & $5\%$ & -- \\
FlexiAct      & $8\%$ & -- \\
DisMo         & $24\%$ & $26\%$ \\
\modelname{}  & $\mathbf{63\%}$ & $\mathbf{74\%}$ \\
\bottomrule
\end{tabular*}
\captionof{table}{\textbf{User study:} share of choices for each method; participants see the source, the target and the generations in random order. \modelname{} on Cog-5B.}
\label{tab:user}

